Unsupervised Resource Allocation with Graph Neural Networks

We present an approach for maximizing a global utility function by learning how to allocate resources in an unsupervised way. We expect interactions between allocation targets to be important and therefore propose to learn the reward structure for near-optimal allocation policies with a GNN. By relaxing the resource constraint, we can employ gradient-based optimization in contrast to more standard evolutionary algorithms. Our algorithm is motivated by a problem in modern astronomy, where one needs to select-based on limited initial information-among $10^9$ galaxies those whose detailed measurement will lead to optimal inference of the composition of the universe. Our technique presents a way of flexibly learning an allocation strategy by only requiring forward simulators for the physics of interest and the measurement process. We anticipate that our technique will also find applications in a range of resource allocation problems.

==> macros.tex <==
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}

\newenvironment{tight_it}{
\begin{itemize}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \setlength{\parsep}{0pt}
}{\end{itemize}}

\newcommand\responsenord[2]{{\color{blue}#1: #2}}
\newcommand\bv{\mathbf{v}}

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother


\newcommand{\mat}[2]{% rows, cols
\vcenter{\hbox{ %Vertical alignment
\begin{tikzpicture}[scale=0.3, align=center]
\filldraw[step=1,black] (0.0, 0.0) grid (#1, #2);
\end{tikzpicture}
}}}

% cols, rows, label
\newcommand{\labmat}[3]{
\stackrel{#3}{
\vcenter{\hbox{ %Vertical alignment
\begin{tikzpicture}[scale=0.2, align=center]
\filldraw[step=1] (0.0, 0.0) grid (#1, #2);
\end{tikzpicture}
}}}}

% cols, rows, rows_shade_start, cols_shade_start, rows_shade_end, cols_shade_end, label
\newcommand{\colormat}[7]{
\stackrel{#7}{
\vcenter{\hbox{ %Vertical alignment
\begin{tikzpicture}[scale=0.3, align=center]
\filldraw[step=1] (0.0, 0.0) grid (#1, #2);
\filldraw[shift={(#3,#4)}, fill=gray] (0, 0) rectangle (#5,#6);
\end{tikzpicture}
}}}}


\setcitestyle{square,numbers}


%\newcommand{\algorithmautorefname}{Algorithm}
\renewcommand{\subsectionautorefname}{Section}


==> packages.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{comment}
\usepackage[normalem]{ulem}
%\usetikzlibrary{matrix,positioning,fit}

\usepackage{amsmath}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}


